DiffPoint: Single and Multi-view Point Cloud Reconstruction with ViT Based Diffusion Model

As the task of 2D-to-3D reconstruction has gained significant attention in various real-world scenarios, it becomes crucial to be able to generate high-quality point clouds. Despite the recent success of deep learning models in generating point clouds, there are still challenges in producing high-fidelity results due to the disparities between images and point clouds. While vision transformers (ViT) and diffusion models have shown promise in various vision tasks, their benefits for reconstructing point clouds from images have not been demonstrated yet. In this paper, we first propose a neat and powerful architecture called DiffPoint that combines ViT and diffusion models for the task of point cloud reconstruction. At each diffusion step, we divide the noisy point clouds into irregular patches. Then, using a standard ViT backbone that treats all inputs as tokens (including time information, image embeddings, and noisy patches), we train our model to predict target points based on input images. We evaluate DiffPoint on both single-view and multi-view reconstruction tasks and achieve state-of-the-art results. Additionally, we introduce a unified and flexible feature fusion module for aggregating image features from single or multiple input images. Furthermore, our work demonstrates the feasibility of applying unified architectures across languages and images to improve 3D reconstruction tasks.

==> tmp/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

\begin{table*}[htbp!]
\centering
\caption{ShapeNet}
\label{tab:exp_abl}
\scalebox{0.8}{
 \begin{tabular}{c|c} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
\toprule[2pt]
    \textbf{Category} & \textbf{Count}\\
\midrule[2pt]
\midrule[2pt]
      Plane  &2831 \\
      Bench  & 1271\\
      Cabinet & 1100\\
      Car & 5247\\
      Chair & 4744\\
      Display  &766 \\
      Lamp  &1622\\
      Loudspeaker  &1132\\
      Rifle &1660\\
      Sofa  &2221\\
      Table &5956\\
      Telephone & 736\\
      Vessel &1357\\
\bottomrule[2pt]
\end{tabular}}
\end{table*}

\item Extensive experimental results demonstrate that our model reconstructs state-of-the-art results in single-view and multi-view 3D shape reconstruction. Additional experiments on OBJAVERSE-LVIS also show its strong modelling capabilities. 


In recent years, there has been significant interest in 2D-to-3D reconstruction in the field of 3D computer vision. The goal of this task is to create a three-dimensional representation of an object using one or more two-dimensional images as input. It finds applications in robotics, autonomous driving, and virtual reality. However, establishing feature correspondences between the images and 3D data is challenging due to their substantial differences. To address these limitations, deep learning models for 3D reconstruction have made significant advancements in terms of quality and flexibility. Existing models can be broadly categorized into three types based on the explicit representation of 3D data: voxel-based models \cite{Choy20163DR2N2AU,Xie2019Pix2VoxC3,Xie2020Pix2VoxMC, Yagubbayli2021LegoFormerTF}, mesh-based models \cite{Wen2022Pixel2Mesh3M,Wang2018Pixel2MeshG3,Pan2019DeepMR}, and point-based models \cite{Wen20223DSR,Fan2017APS}. While voxel-based representations suffer from high memory costs at high resolutions, meshes struggle to produce accurate results with inner or irregular structures despite being widely used in gaming. On the other hand, point clouds offer lightweight storage consumption and are capable of representing various complex shapes compared to these previous forms of 3D shape representation. 
\par

Though these methods achieve some success to some extent, the 2D-to-3D reconstruction task is still suffering from the following problem: how to find an effective way to reduce the disparities between images and 3D shapes for reconstructing accurate results. Most previous methods \cite{Choy20163DR2N2AU,Xie2019Pix2VoxC3,Xie2020Pix2VoxMC, Yagubbayli2021LegoFormerTF, Wen2022Pixel2Mesh3M,Wang2018Pixel2MeshG3,Pan2019DeepMR } follows the standard encoder-decoder structure, in which image features are treated as additional information and limited semantic information can be conveyed to the 3D decoder. Limited by the modeling ability, as a result, these methods fail to reconstruct satisfactory results, especially reconstructing objects with complex structure. 
Driven by scaling models on large datasets, diffusion models \cite{SohlDickstein2015DeepUL,Ho2020DenoisingDP,Song2020ScoreBasedGM} have shown great success in various tasks \cite{Nichol2022GLIDETP,Dhariwal2021DiffusionMB,Tashiro2021CSDICS,Kong2021DiffWaveAV,Kim2022GuidedTTSAD, Radford2021LearningTV}. Diffusion models have emerged as highly effective generative models, showcasing exceptional performance in not only image synthesis \cite{Ramesh2022HierarchicalTI, Chang2023MuseTG, Dhariwal2021DiffusionMB, Preechakul2021DiffusionAT,Rombach2021HighResolutionIS} but also the generation of 3D shapes based on point clouds \cite{Luo2021DiffusionPM,Zeng2022LIONLP,Zhou20213DSG,Mo2023DiT3DEP}. Diffusion models show potential to be able to be adopted for 3D reconstruction. However, existing point-based diffusion models cannot perfectly solve the problem above. With a backbone implemented by MLP \cite{Luo2021DiffusionPM} and PVCNN \cite{ Zeng2022LIONLP,Zhou20213DSG },  they also treat the image embedding as addition al information, failing to fully explore the visual information. Moreover, DPM based on MLP fail to reconstruct complex structure shapes. For Point-Voxel CNN (PVCNN) based diffusion models \cite{Zeng2022LIONLP,Zhou20213DSG}, they requires huge memory and computation costs to implement voxel convolution operation. On the other hand, vision transformers (ViT) \cite{Dosovitskiy2020AnII} have shown promise in various vision tasks with a flexibility backbone. As point cloud essentially shares a common property with languages and images, a very natural question arises: can ViT be adapted to diffusion models for point cloud reconstruction tasks? Combining diffusion models with ViT may address the problem above: a) The ViT backbone in diffusion models helps in creating a more expressive and context-aware representation of features, in which hierarchical attention mechanisms of ViT capture both global and local information effectively; b) ViT's token-based approach allows for the assimilation of diverse information, including time, image embeddings, and patches, enabling the model to bridge the gap between different modalities effectively.
\par

In this paper, we propose DiffPoint, a robost and flexible ViT-based diffusion architecture for point cloud reconstruction. Directly extending ViT and diffusion models to point cloud is, however, technically highly nontrivial: different from images, point clouds are composed of discrete points in the 3D space, which means that point clouds cannot be directly divided into patches as images. To address the problem above, we follow the design methodology of PointMAE \cite{Pang2022MaskedAF} and Point-BERT \cite{Yu2021PointBERTP3}, where point cloud are divided into irregular patches through Farthest Point Sampling (FPS) and K-Nearest Neighborhood (KNN) algorithm. Then the divided patches are encoded to token embedding with a lightweight encoder PointNet \cite{Qi2016PointNetDL}. As CLIP \cite{Radford2021LearningTV} have been shown to learn robust representations of images that capture both semantics and style, we leverage these representations to point cloud reconstruction. The input images are encoded with CLIP to image embedding. In order to reduce the gap between images and point clouds, we also, same as U-ViT \cite{Bao2022AllAW}, treat all inputs including the time, image embedding, noisy points patches as tokens, in which images embedding and points embedding make a feature interaction in the same space. Besides, to maintain the consistency and flexibility of the model architecture, we design a multi feature aggregation module for single and multi-view tasks, which can aggregate features from single or multi input images.
\par

We evaluate our DiffPoint in single and multi-view reconstruction tasks. Our results on popular benchmark ShapeNet \cite{Chang2015ShapeNetAI} suggests that DiffPoint is capable of reconstruct high-fidelity point clouds, outperforming multiple state-of-the-art methods. Beyond that, we extend DiffPoint to a more complicated and diverse dataset OBJAVERSE-LVIS \cite{Deitke2022ObjaverseAU}, demonstrating the powerful modelling capabilities of DiffPoint and the potential to migrate to large-scale 3D datasets.
\par

The main contributions of this paper are summarized as follows:
\begin{itemize}
    \item We study the 3D point cloud reconstruction task and propose a novel framework based on a denoising diffusion models and ViT, called DiffPoint. To the best of our knowledge, this is the first attempt that employs ViT based diffusion models  in the 3D point cloud reconstruction task. 
    \item We propose a unified multi feature aggregation module for single and multi-view reconstruction tasks, keeping consistency in the model architecture across both tasks.
    \item Extensive experimental results demonstrate that our model reconstructs state-of-the-art results in single-view and multi-view 3D shape reconstruction. Additional experiments on OBJAVERSE-LVIS also show its strong modelling capabilities. 
\end{itemize}



\section{Introduction}
\label{sec:intro}

In recent years, there has been significant interest in 2D-to-3D reconstruction in the field of 3D computer vision. The goal of this task is to create a three-dimensional representation of an object using one or more two-dimensional images as input. It finds applications in robotics, autonomous driving, and virtual reality. However, establishing feature correspondences between the images and 3D data is challenging due to their substantial differences. To address these limitations, deep learning models for 3D reconstruction have made significant advancements in terms of quality and flexibility. Existing models can be broadly categorized into three types based on the explicit representation of 3D data: voxel-based models \cite{Choy20163DR2N2AU,Xie2019Pix2VoxC3,Xie2020Pix2VoxMC, Yagubbayli2021LegoFormerTF}, mesh-based models \cite{Wen2022Pixel2Mesh3M,Wang2018Pixel2MeshG3,Pan2019DeepMR}, and point-based models \cite{Wen20223DSR,Fan2017APS}. While voxel-based representations suffer from high memory costs at high resolutions, meshes struggle to produce accurate results with inner or irregular structures despite being widely used in gaming. On the other hand, point clouds offer lightweight storage consumption and are capable of representing various complex shapes compared to these previous forms of 3D shape representation. Though these methods achieve some success to some extent, the 2D-to-3D reconstruction task is still suffering from the following problems: a) A robust model for achieving satisfactory results on 3D dataset; b) A flexible backbone that can balance modeling capability and computational costs.
\par

Driven by scaling models on large datasets, diffusion models \cite{SohlDickstein2015DeepUL,Ho2020DenoisingDP,Song2020ScoreBasedGM} have shown great success in various tasks \cite{Nichol2022GLIDETP,Dhariwal2021DiffusionMB,Tashiro2021CSDICS,Kong2021DiffWaveAV,Kim2022GuidedTTSAD, Radford2021LearningTV}. Diffusion models have emerged as highly effective generative models, showcasing exceptional performance in not only image synthesis \cite{Ramesh2022HierarchicalTI, Chang2023MuseTG, Dhariwal2021DiffusionMB, Preechakul2021DiffusionAT,Rombach2021HighResolutionIS} but also the generation of 3D shapes based on point clouds \cite{Luo2021DiffusionPM,Zeng2022LIONLP,Zhou20213DSG,Mo2023DiT3DEP}. Initialized from random noise, diffusion models capture the data distribution through a Markov chain to convert the noise distribution to the data distribution. Existing point-based diffusion models, focusing on the unconditional and class-conditional point generation task, struggle with low modelling capability or huge memory costs. DPM \cite{Luo2021DiffusionPM} with a simple backbone implemented by MLP fail to reconstruct complex structure shapes. For Point-Voxel CNN (PVCNN) based diffusion models \cite{Zeng2022LIONLP,Zhou20213DSG}, they requires huge memory and computation costs to implement voxel convolution operation. On the other hand, vision transformers (ViT) \cite{Dosovitskiy2020AnII} have shown promise in various vision tasks with a flexibility backbone. As point cloud essentially shares a common property with languages and images, a very natural question arises: can ViT be adapted to diffusion models for point cloud reconstruction tasks?
\par

Inspired by the diffusion model and ViT scaling success in images, we propose DiffPoint, a robost and flexible ViT-based diffusion architecture for point cloud reconstruction. Also, ViT is able to flexibly adjust the complexity of the backbone network according to the scale of the dataset. Combining diffusion models with ViT may address 2D-to-3D reconstruction problems above. Directly extending ViT and diffusion models to point cloud is, however, technically highly nontrivial: different from images, point clouds are composed of discrete points in the 3D space, which means that point clouds cannot be directly divided into patches as images. To address the problem above, we follow the design methodology of PointMAE \cite{Pang2022MaskedAF} and Point-BERT \cite{Yu2021PointBERTP3}, where point cloud are divided into irregular patches through Farthest Point Sampling (FPS) and K-Nearest Neighborhood (KNN) algorithm. Then the divided patches are encoded to token embedding with a lightweight encoder PointNet \cite{Qi2016PointNetDL}. As CLIP \cite{Radford2021LearningTV} have been shown to learn robust representations of images that capture both semantics and style, we leverage these representations to point cloud reconstruction. The input images are encoded with CLIP to image embedding. In order to reduce the gap between images and point clouds, we also, same as U-ViT \cite{Bao2022AllAW}, treat all inputs including the time, image embedding, noisy points patches as tokens, in which images embedding and points embedding make a feature interaction in the same space. Besides, to maintain the consistency and flexibility of the model architecture, we design a multi feature aggregation module for single and multi-view tasks, which can aggregate features from single or multi input images.
\par

We evaluate our DiffPoint in single and multi-view reconstruction tasks. Our results on popular benchmark ShapeNet \cite{Chang2015ShapeNetAI} suggests that DiffPoint is capable of reconstruct high-fidelity point clouds, outperforming multiple state-of-the-art methods. Beyond that, we extend DiffPoint to a more complicated and diverse dataset OBJAVERSE-LVIS \cite{Deitke2022ObjaverseAU}, demonstrating the powerful modelling capabilities of DiffPoint and the potential to migrate to large-scale 3D datasets.
\par

The main contributions of this paper are summarized as follows:
\begin{itemize}
    \item We study the 3D point cloud reconstruction task and propose a novel framework based on a denoising diffusion models and ViT, called DiffPoint. To the best of our knowledge, this is the first attempt that employs ViT based diffusion models  in the 3D point cloud reconstruction task. 
    \item We propose a unified multi feature aggregation module for single and multi-view reconstruction tasks, keeping consistency in the model architecture across both tasks.
    \item Extensive experimental results demonstrate that our model reconstructs state-of-the-art results in single-view and multi-view 3D shape reconstruction. Additional experiments on OBJAVERSE-LVIS also show its strong modelling capabilities. 
\end{itemize}

While ViT is excellent at capturing global context, it may struggle with capturing fine-grained local details in images. 3D point cloud reconstruction often requires precise information about individual points, and ViT might not be as effective in this regard compared to architectures specifically designed for point cloud processing.

==> tmp/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> tmp/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
